Active Information Gathering for Long-Horizon Navigation Under Uncertainty by Learning the Value of Information

We address the task of long-horizon navigation in partially mapped environments for which active gathering of information about faraway unseen space is essential for good behavior. We present a novel planning strategy that, at training time, affords tractable computation of the value of information associated with revealing potentially informative regions of unseen space, data used to train a graph neural network to predict the goodness of temporally-extended exploratory actions. Our learning-augmented model-based planning approach predicts the expected value of information of revealing unseen space and is capable of using these predictions to actively seek information and so improve long-horizon navigation. Across two simulated office-like environments, our planner outperforms competitive learned and non-learned baseline navigation strategies, achieving improvements of up to 63.76% and 36.68%, demonstrating its capacity to actively seek performance-critical information.

==> 10_preliminaries.tex <==
\begin{figure}[t]
  \includegraphics[width=.48\textwidth]{figures/explain-lsp-action.png}
    \caption{
    \textbf{Our robot's actions correspond to boundaries between free and unseen space.}
    The robot can leave observed space through either boundary: via subgoal $s_1$ or $s_2$. Upon selecting action $a_2$, the robot reaches the goal with probability $P_S$ and incurs an expected cost $R_S$, or is turned back (probability $1-P_S$), accumulates cost $R_E$ and selects another action.
    }
  \label{fig:lsp-example}
\end{figure}

\section{Preliminaries: Model-based Planning under Uncertainty via Learning over Subgoals}
\label{sec:lsp}
As Eq.~\eqref{eq:POMDP} cannot be solved directly, our robot instead relies on the recent Learning over Subgoals Planning (LSP) approach~\cite{pmlr-v87-stein18a} to determine the robot's behavior.
LSP introduces a model-based planning abstraction that alleviates the computational requirements of POMDP planning, affording both reliability and good performance informed by predictions about unseen space from learning.

For LSP planning as described in Fig.~\ref{fig:lsp-example}, actions available to the robot correspond to navigation to \emph{subgoals}---each associated with a boundary between free and unknown space---and then exploration beyond in an effort to reach the unseen goal.
Consistent with this action abstraction, planning under the LSP model is done over an abstract belief state: a tuple $b_t = \{m_t, q_t\}$, where $m_t$ is the current map of the environment, and $q_t$ is the robot pose.
Each high-level action $a_t \in \mathcal{A}(\{m_t, q_t\})$ has a binary outcome: with probability $P_S(a_t)$, the robot \emph{succeeds} in reaching the goal or (with the inverse probability $1 - P_S(a_t)$) fails to reach the goal.
Upon selecting an action $a_t$, the robot must first move through known space to the boundary, accumulating a cost $D(m_t, q_t, a_t)$.
If the robot succeeds in reaching the goal, it accumulates a \emph{success cost} $R_S(a_t)$, the expected cost for the robot to reach the goal, and no further navigation is necessary.
Otherwise, the robot accumulates an \emph{exploration cost} $R_E(a_t)$, the expected cost of exploring the region beyond the subgoal of interest and needing to turn back, and must subsequently choose another action $a_{t+1} \in A_{t+1} \equiv \mathcal{A}(\{m_t, q(a_t)\})\setminus \{ a_t \}$.

Under this LSP planning model, the expected cost of taking an action $a_t$ from belief state $b_t = \{ m_t, q_t\}$ is
\begin{equation}\label{eq:lsp-planning}
\begin{split}
    Q(&\{m_t, q_t\}, a_t\in  \mathcal{A}) = D(m_t, q_t, a_t) + P_S(a_t) R_S(a_t) \\
    & + (1-P_S(a_t)) \left[R_E(a_t) + \min_{a_{t+1}}Q(\{m_t, q(a_t)\},a_{t+1}) \right]
    \end{split}
\end{equation}
While the known-space distance $D(m_t, q_t, a_t)$ can be calculated directly from the observed map using A$^{\!*}$ or RRT$^*$, the \emph{subgoal properties} $P_S(a_t)$, $R_S(a_t)$, and $R_E(a_t)$ for each subgoal are estimated via learning from information collected during navigation.\footnote{The terms $P_S$, $R_S$, and $R_E$ are implicitly functions of the belief, but shown here only as functions of the chosen action for notational simplicity.}
We use the LSP-GNN strategy of Arnob and Stein~\cite{arnob2023lspgnn}, in which a graph neural network~\cite{peter2018} is used to estimate the subgoal properties, using a graphical representation of the entire map to make predictions.
However, this approach does not reason about the value of information for revealing a particular part of the environment.
% approach cannot reason about the value of information for the unseen spaces and cannot use it to plan.
We show an example of this limitation in Sec.~\ref{sec:example-case} and discuss how we overcome it via our approach in Sec.~\ref{sec:eq-theory-value-of-info}.

